ModelGuard: Runtime Validation of Lipschitz-continuous Models

This paper presents ModelGuard, a sampling-based approach to runtime model validation for Lipschitz-continuous models. Although techniques exist for the validation of many classes of models the majority of these methods cannot be applied to the whole of Lipschitz-continuous models, which includes neural network models. Additionally, existing techniques generally consider only white-box models. By taking a sampling-based approach, we can address black-box models, represented only by an input-output relationship and a Lipschitz constant. We show that by randomly sampling from a parameter space and evaluating the model, it is possible to guarantee the correctness of traces labeled consistent and provide a confidence on the correctness of traces labeled inconsistent. We evaluate the applicability and scalability of ModelGuard in three case studies, including a physical platform.

==> Weimer_defs.tex <==
% !TEX root = root.tex

%% Jim's definitions and use packages
%
\graphicspath{{figs/}}
%
%% General packages
%%\usepackage{graphicx}
\usepackage{paralist}
\usepackage{color}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{bm} % for bold symbols like \bm{\alpha} or {\bm \alpha\beta}
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Jim's commands
%
%% Labels, equations, matrices
\newcommand{\eqnref}			[1]		{Equation~\ref{eqn:#1}}
\newcommand{\tableref}			[1]		{Table~\ref{tab:#1}}
\newcommand{\figref}			[1]		{Figure~\ref{fig:#1}}
\newcommand{\eqa}				[1]		{\begin{eqnarray}#1\end{eqnarray}}
\newcommand{\eqs}				[1]		{\begin{equation*}\begin{split}#1\end{split}\end{equation*}}
\newcommand{\eq}				[1]		{\begin{equation}\begin{split}#1\end{split}\end{equation}}
\newcommand{\eqsub}			[1]		{\begin{subequations}\begin{align}#1\end{align}\end{subequations}}
\newcommand{\mat}				[2]		{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\arr}				[2]		{\begin{array}{#1} #2 \end{array}}
\newcommand{\inv}				[1]		{\left( #1 \right)^{-1}}
\newcommand{\abs}				[1]		{\left| #1 \right|}
%
%
%% mathematical names
%\newcommand{\bernoulli}					{\mathrm{bernoulli}}
%\newcommand{\erf}				[1]		{\mathrm{erf}\left(#1\right)}
\newcommand{\diag}				[1]		{\mathrm{diag}\left(#1\right)}
%
%
%% Number types
\newcommand{\realnum}					{\mathbb{R}}
%\newcommand{\complexnum}				{\mathbb{C}}
\newcommand{\naturalnum}				{\mathbb{N}}
%
%
%% Common mathematical functions and symbols
\newcommand{\Exp}		[1]		{\mathbb{E}\left[#1\right]}
\newcommand{\ExpOf}	[2]		{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\Var}		[1]		{\mathrm{Var}\left[#1\right]}
\newcommand{\Cov}		[1]		{\mathrm{Cov}\left[#1\right]}
\newcommand{\CovarianceOf}		[1]		{\mathrm{Cov}\left[#1\right]}
%\newcommand{\CovarianceOfx}	[2]		{\mathrm{Cov}_{#1}\left[#2\right]}
\newcommand{\var}		[1]		{\mathrm{var}\left[#1\right]}
\newcommand{\VarianceOf}		[1]		{\mathrm{var}\left[#1\right]}
%\newcommand{\VarianceOfx}	[2]		{\mathrm{var}_{#1}\left[#2\right]}
%\newcommand{\TraceOf}			[1]		{\mathrm{Tr}\left[#1\right]}
%\newcommand{\RankOf}			[1]		{\mathrm{rank}\left(#1\right)}
\newcommand{\ProbabilityOf}		[1]		{\mathrm{Pr}\left[#1\right]}
\newcommand{\Prob}			[1]		{\mathrm{Pr}\left[#1\right]}
%\newcommand{\SpanOf}			[1]		{\mathrm{span} \left\langle #1 \right\rangle}
%\newcommand{\DefinedAs}		[0]		{\mathrel{\mathop:}=}
%\newcommand{\zeros}			[0]		{\mathbf{0}}
%\newcommand{\set}				[1]		{\left\{#1\right\}}
%\newcommand{\bmv}				[1]		{\boldsymbol{\mathrm{#1}}}
%%\newcommand{\qedhere}		{\hfill \ensuremath{\Box}}
%\newcommand{\Ind}				[1]  		{\mathcal{I}\left(#1\right)}
\renewcommand{\(}						{\left(}
\renewcommand{\)}						{\right)}
\renewcommand{\[}						{\left[}
\renewcommand{\]}						{\right]}
\newcommand{\<}						{\left<}
\renewcommand{\>}						{\right>}

\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\asteq}{\mathrel{*}=}

\newcommand{\nullspaceOf}		[1]		{\left< #1 \right>^{\perp}}
\newcommand{\spaceOf}			[1]		{\left< #1 \right>}

\newcommand{\nullspace}			[1]		{Null\left( #1 \right)}
\newcommand{\image}			[1]		{Im\left( #1 \right)}
%\newcommand{\and}						{\wedge}
%\newcommand{\or}						{\vee}
%
%% Other commands
%%\newcommand{\bm}	[1]	{\boldsymbol{#1}}
%
%
%\newcommand{\Expe}[1]{\bm{\mathrm{e}}^{#1}}
%\def\precise{{\sc Precise~}}
%

\newcommand{\ie}{\emph{i.e.,}~}
\newcommand{\eg}{\emph{e.g.,}~}

\newcommand{\err}{\mathrm{err}}
\newcommand{\errh}{\hat{\mathrm{err}}}


\newcommand{\inp}[2]{ \left< #1 , #2 \right>}


\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{problem}{Problem}
\newtheorem{remark}{Remark}








%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Jim's alphabet definitions
%
%
%% bold lower case
\def\a{\bm{a}}
\def\b{\bm{b}}
\def\c{\bm{c}}
\def\d{\bm{d}}
\def\e{\bm{e}}
\def\f{\bm{f}}
\def\g{\bm{g}}
\def\h{\bm{h}}
%\def\i{\bm{i}}
\def\j{\bm{j}}
\def\k{\bm{k}}
\def\l{\bm{l}}
\def\m{\bm{m}}
\def\n{\bm{n}}
%\def\o{\bm{o}}
\def\p{\bm{p}}
\def\q{\bm{q}}
\def\r{\bm{r}}
\def\s{\bm{s}}
\def\t{\bm{t}}
\def\u{\bm{u}}
\def\v{\bm{v}}
\def\w{\bm{w}}
\def\x{\bm{x}}
\def\y{\bm{y}}
\def\z{\bm{z}}
\def\A{\bm{A}}
\def\B{\bm{B}}
\def\C{\bm{C}}
\def\D{\bm{D}}
\def\E{\bm{E}}
\def\F{\bm{F}}
\def\G{\bm{G}}
\def\H{\bm{H}}
\def\I{\bm{I}}
\def\J{\bm{J}}
\def\K{\bm{K}}
\def\L{\bm{L}}
\def\M{\bm{M}}
\def\N{\bm{N}}
\def\O{\bm{O}}
\def\P{\bm{P}}
\def\Q{\bm{Q}}
\def\R{\bm{R}}
\def\S{\bm{S}}
\def\T{\bm{T}}
\def\U{\bm{U}}
\def\V{\bm{V}}
\def\W{\bm{W}}
\def\X{\bm{X}}
\def\Y{\bm{Y}}
\def\Z{\bm{Z}}
\def\Beta{\bm{\beta}}
%
%
%
%% bold hat
\def\aH{\hat{\bm{a}}}
\def\bH{\hat{\bm{b}}}
\def\cH{\hat{\bm{c}}}
\def\dH{\hat{\bm{d}}}
\def\eH{\hat{\bm{e}}}
\def\fH{\hat{\bm{f}}}
\def\gH{\hat{\bm{g}}}
\def\hH{\hat{\bm{h}}}
\def\iH{\hat{\bm{i}}}
\def\iH{\hat{\bm{j}}}
\def\kH{\hat{\bm{k}}}
\def\lH{\hat{\bm{l}}}
\def\mH{\hat{\bm{m}}}
\def\nH{\hat{\bm{n}}}
\def\oH{\hat{\bm{o}}}
\def\pH{\hat{\bm{p}}}
\def\qH{\hat{\bm{q}}}
\def\rH{\hat{\bm{r}}}
\def\sH{\hat{\bm{s}}}
\def\tH{\hat{\bm{t}}}
\def\uH{\hat{\bm{u}}}
\def\vH{\hat{\bm{v}}}
\def\wH{\hat{\bm{w}}}
\def\xH{\hat{\bm{x}}}
\def\yH{\hat{\bm{y}}}
\def\zH{\hat{\bm{z}}}
\def\AH{\hat{\bm{A}}}
\def\BH{\hat{\bm{B}}}
\def\CH{\hat{\bm{C}}}
\def\DH{\hat{\bm{D}}}
\def\EH{\hat{\bm{E}}}
\def\FH{\hat{\bm{F}}}
\def\GH{\hat{\bm{G}}}
\def\HH{\hat{\bm{H}}}
\def\IH{\hat{\bm{I}}}
\def\JH{\hat{\bm{J}}}
\def\KH{\hat{\bm{K}}}
\def\LH{\hat{\bm{L}}}
\def\MH{\hat{\bm{M}}}
\def\NH{\hat{\bm{N}}}
\def\OH{\hat{\bm{O}}}
\def\PH{\hat{\bm{P}}}
\def\QH{\hat{\bm{Q}}}
\def\RH{\hat{\bm{R}}}
\def\SH{\hat{\bm{S}}}
\def\TH{\hat{\bm{T}}}
\def\UH{\hat{\bm{U}}}
\def\VH{\hat{\bm{V}}}
\def\WH{\hat{\bm{W}}}
\def\XH{\hat{\bm{X}}}
\def\YH{\hat{\bm{Y}}}
\def\ZH{\hat{\bm{Z}}}
%
% bold bar
\def\aB{\bar{\bm{a}}}
\def\bB{\bar{\bm{b}}}
\def\cB{\bar{\bm{c}}}
\def\dB{\bar{\bm{d}}}
\def\eB{\bar{\bm{e}}}
\def\fB{\bar{\bm{f}}}
\def\gB{\bar{\bm{g}}}
\def\hB{\bar{\bm{h}}}
\def\iB{\bar{\bm{i}}}
\def\iB{\bar{\bm{j}}}
\def\kB{\bar{\bm{k}}}
\def\lB{\bar{\bm{l}}}
\def\mB{\bar{\bm{m}}}
\def\nB{\bar{\bm{n}}}
\def\oB{\bar{\bm{o}}}
\def\pB{\bar{\bm{p}}}
\def\qB{\bar{\bm{q}}}
\def\rB{\bar{\bm{r}}}
\def\sB{\bar{\bm{s}}}
\def\tB{\bar{\bm{t}}}
\def\uB{\bar{\bm{u}}}
\def\vB{\bar{\bm{v}}}
\def\wB{\bar{\bm{w}}}
\def\xB{\bar{\bm{x}}}
\def\yB{\bar{\bm{y}}}
\def\zB{\bar{\bm{z}}}
\def\AB{\bar{\bm{A}}}
\def\BB{\bar{\bm{B}}}
\def\CB{\bar{\bm{C}}}
\def\DB{\bar{\bm{D}}}
\def\EB{\bar{\bm{E}}}
\def\FB{\bar{\bm{F}}}
\def\GB{\bar{\bm{G}}}
\def\HB{\bar{\bm{H}}}
\def\IB{\bar{\bm{I}}}
\def\JB{\bar{\bm{J}}}
\def\KB{\bar{\bm{K}}}
\def\LB{\bar{\bm{L}}}
\def\MB{\bar{\bm{M}}}
\def\NB{\bar{\bm{N}}}
\def\OB{\bar{\bm{O}}}
\def\PB{\bar{\bm{P}}}
\def\QB{\bar{\bm{Q}}}
\def\RB{\bar{\bm{R}}}
\def\SB{\bar{\bm{S}}}
\def\TB{\bar{\bm{T}}}
\def\UB{\bar{\bm{U}}}
\def\VB{\bar{\bm{V}}}
\def\WB{\bar{\bm{W}}}
\def\XB{\bar{\bm{X}}}
\def\YB{\bar{\bm{Y}}}
\def\ZB{\bar{\bm{Z}}}
%
%%% bold tilde
%%\def\aT{\tilde{\bm{a}}}
%%\def\bT{\tilde{\bm{b}}}
%%\def\cT{\tilde{\bm{c}}}
%%\def\dT{\tilde{\bm{d}}}
%%\def\eT{\tilde{\bm{e}}}
%%\def\fT{\tilde{\bm{f}}}
%%\def\gT{\tilde{\bm{g}}}
%%\def\hT{\tilde{\bm{h}}}
%%\def\iT{\tilde{\bm{i}}}
%%\def\iT{\tilde{\bm{j}}}
%%\def\kT{\tilde{\bm{k}}}
%%\def\lT{\tilde{\bm{l}}}
%%\def\mT{\tilde{\bm{m}}}
%%\def\nT{\tilde{\bm{n}}}
%%\def\oT{\tilde{\bm{o}}}
%%\def\pT{\tilde{\bm{p}}}
%%\def\qT{\tilde{\bm{q}}}
%%\def\rT{\tilde{\bm{r}}}
%%\def\sT{\tilde{\bm{s}}}
%%\def\tT{\tilde{\bm{t}}}
%%\def\uT{\tilde{\bm{u}}}
%%\def\vT{\tilde{\bm{v}}}
%%\def\wT{\tilde{\bm{w}}}
%%\def\xT{\tilde{\bm{x}}}
%%\def\yT{\tilde{\bm{y}}}
%%\def\zT{\tilde{\bm{z}}}
%%\def\AT{\tilde{\bm{A}}}
%%\def\BT{\tilde{\bm{B}}}
%%\def\CT{\tilde{\bm{C}}}
%%\def\DT{\tilde{\bm{D}}}
%%\def\ET{\tilde{\bm{E}}}
%%\def\FT{\tilde{\bm{F}}}
%%\def\GT{\tilde{\bm{G}}}
%%\def\HT{\tilde{\bm{H}}}
%%\def\IT{\tilde{\bm{I}}}
%%\def\JT{\tilde{\bm{J}}}
%%\def\KT{\tilde{\bm{K}}}
%%\def\LT{\tilde{\bm{L}}}
%%\def\MT{\tilde{\bm{M}}}
%%\def\NT{\tilde{\bm{N}}}
%%\def\OT{\tilde{\bm{O}}}
%%\def\PT{\tilde{\bm{P}}}
%%\def\QT{\tilde{\bm{Q}}}
%%\def\RT{\tilde{\bm{R}}}
%%\def\ST{\tilde{\bm{S}}}
%%\def\TT{\tilde{\bm{T}}}
%%\def\UT{\tilde{\bm{U}}}
%%\def\VT{\tilde{\bm{V}}}
%%\def\WT{\tilde{\bm{W}}}
%%\def\XT{\tilde{\bm{X}}}
%%\def\YT{\tilde{\bm{Y}}}
%%\def\ZT{\tilde{\bm{Z}}}
%
%% bold vec
%\def\aV{\vec{\bm{a}}}
%\def\bV{\vec{\bm{b}}}
%\def\cV{\vec{\bm{c}}}
%\def\dV{\vec{\bm{d}}}
%\def\eV{\vec{\bm{e}}}
%\def\fV{\vec{\bm{f}}}
%\def\gV{\vec{\bm{g}}}
%\def\hV{\vec{\bm{h}}}
%\def\iV{\vec{\bm{i}}}
%\def\iV{\vec{\bm{j}}}
%\def\kV{\vec{\bm{k}}}
%\def\lV{\vec{\bm{l}}}
%\def\mV{\vec{\bm{m}}}
%\def\nV{\vec{\bm{n}}}
%\def\oV{\vec{\bm{o}}}
%\def\pV{\vec{\bm{p}}}
%\def\qV{\vec{\bm{q}}}
%\def\rV{\vec{\bm{r}}}
%\def\sV{\vec{\bm{s}}}
%\def\tV{\vec{\bm{t}}}
%\def\uV{\vec{\bm{u}}}
%\def\vV{\vec{\bm{v}}}
%\def\wV{\vec{\bm{w}}}
%\def\xV{\vec{\bm{x}}}
%\def\yV{\vec{\bm{y}}}
%\def\zV{\vec{\bm{z}}}
%\def\AV{\vec{\bm{A}}}
%\def\BV{\vec{\bm{B}}}
%\def\CV{\vec{\bm{C}}}
%\def\DV{\vec{\bm{D}}}
%\def\EV{\vec{\bm{E}}}
%\def\FV{\vec{\bm{F}}}
%\def\GV{\vec{\bm{G}}}
%\def\HV{\vec{\bm{H}}}
%\def\IV{\vec{\bm{I}}}
%\def\JV{\vec{\bm{J}}}
%\def\KV{\vec{\bm{K}}}
%\def\LV{\vec{\bm{L}}}
%\def\MV{\vec{\bm{M}}}
%\def\NV{\vec{\bm{N}}}
%\def\OV{\vec{\bm{O}}}
%\def\PV{\vec{\bm{P}}}
%\def\QV{\vec{\bm{Q}}}
%\def\RV{\vec{\bm{R}}}
%\def\SV{\vec{\bm{S}}}
%\def\TV{\vec{\bm{T}}}
%\def\UV{\vec{\bm{U}}}
%\def\VV{\vec{\bm{V}}}
%\def\WV{\vec{\bm{W}}}
%\def\XV{\vec{\bm{X}}}
%\def\YV{\vec{\bm{Y}}}
%\def\ZV{\vec{\bm{Z}}}
%
%% bold acute
%\def\aA{\acute{\bm{a}}}
%\def\bA{\acute{\bm{b}}}
%\def\cA{\acute{\bm{c}}}
%\def\dA{\acute{\bm{d}}}
%\def\eA{\acute{\bm{e}}}
%\def\fA{\acute{\bm{f}}}
%\def\gA{\acute{\bm{g}}}
%\def\hA{\acute{\bm{h}}}
%\def\iA{\acute{\bm{i}}}
%\def\iA{\acute{\bm{j}}}
%\def\kA{\acute{\bm{k}}}
%\def\lA{\acute{\bm{l}}}
%\def\mA{\acute{\bm{m}}}
%\def\nA{\acute{\bm{n}}}
%\def\oA{\acute{\bm{o}}}
%\def\pA{\acute{\bm{p}}}
%\def\qA{\acute{\bm{q}}}
%\def\rA{\acute{\bm{r}}}
%\def\sA{\acute{\bm{s}}}
%\def\tA{\acute{\bm{t}}}
%\def\uA{\acute{\bm{u}}}
%\def\vA{\acute{\bm{v}}}
%\def\wA{\acute{\bm{w}}}
%\def\xA{\acute{\bm{x}}}
%\def\yA{\acute{\bm{y}}}
%\def\zA{\acute{\bm{z}}}
%\def\AA{\acute{\bm{A}}}
%\def\BA{\acute{\bm{B}}}
%\def\CA{\acute{\bm{C}}}
%\def\DA{\acute{\bm{D}}}
%\def\EA{\acute{\bm{E}}}
%\def\FA{\acute{\bm{F}}}
%\def\GA{\acute{\bm{G}}}
%\def\HA{\acute{\bm{H}}}
%\def\IA{\acute{\bm{I}}}
%\def\JA{\acute{\bm{J}}}
%\def\KA{\acute{\bm{K}}}
%\def\LA{\acute{\bm{L}}}
%\def\MA{\acute{\bm{M}}}
%\def\NA{\acute{\bm{N}}}
%\def\OA{\acute{\bm{O}}}
%\def\PA{\acute{\bm{P}}}
%\def\QA{\acute{\bm{Q}}}
%\def\RA{\acute{\bm{R}}}
%\def\SA{\acute{\bm{S}}}
%\def\TA{\acute{\bm{T}}}
%\def\UA{\acute{\bm{U}}}
%\def\VA{\acute{\bm{V}}}
%\def\WA{\acute{\bm{W}}}
%\def\XA{\acute{\bm{X}}}
%\def\YA{\acute{\bm{Y}}}
%\def\ZA{\acute{\bm{Z}}}
%
%% bold check
%\def\aC{\check{\bm{a}}}
%\def\bC{\check{\bm{b}}}
%\def\cC{\check{\bm{c}}}
%\def\dC{\check{\bm{d}}}
%\def\eC{\check{\bm{e}}}
%\def\fC{\check{\bm{f}}}
%\def\gC{\check{\bm{g}}}
%\def\hC{\check{\bm{h}}}
%\def\iC{\check{\bm{i}}}
%\def\iC{\check{\bm{j}}}
%\def\kC{\check{\bm{k}}}
%\def\lC{\check{\bm{l}}}
%\def\mC{\check{\bm{m}}}
%\def\nC{\check{\bm{n}}}
%\def\oC{\check{\bm{o}}}
%\def\pC{\check{\bm{p}}}
%\def\qC{\check{\bm{q}}}
%\def\rC{\check{\bm{r}}}
%\def\sC{\check{\bm{s}}}
%\def\tC{\check{\bm{t}}}
%\def\uC{\check{\bm{u}}}
%\def\vC{\check{\bm{v}}}
%\def\wC{\check{\bm{w}}}
%\def\xC{\check{\bm{x}}}
%\def\yC{\check{\bm{y}}}
%\def\zC{\check{\bm{z}}}
%\def\AC{\check{\bm{A}}}
%\def\BC{\check{\bm{B}}}
%\def\CC{\check{\bm{C}}}
%\def\DC{\check{\bm{D}}}
%\def\EC{\check{\bm{E}}}
%\def\FC{\check{\bm{F}}}
%\def\GC{\check{\bm{G}}}
%\def\HC{\check{\bm{H}}}
%\def\IC{\check{\bm{I}}}
%\def\JC{\check{\bm{J}}}
%\def\KC{\check{\bm{K}}}
%\def\LC{\check{\bm{L}}}
%\def\MC{\check{\bm{M}}}
%\def\NC{\check{\bm{N}}}
%\def\OC{\check{\bm{O}}}
%\def\PC{\check{\bm{P}}}
%\def\QC{\check{\bm{Q}}}
%\def\RC{\check{\bm{R}}}
%\def\SC{\check{\bm{S}}}
%\def\TC{\check{\bm{T}}}
%\def\UC{\check{\bm{U}}}
%\def\VC{\check{\bm{V}}}
%\def\WC{\check{\bm{W}}}
%\def\XC{\check{\bm{X}}}
%\def\YC{\check{\bm{Y}}}
%\def\ZC{\check{\bm{Z}}}
%
%
%% bold dot
%\def\aD{\dot{\bm{a}}}
%\def\bD{\dot{\bm{b}}}
%\def\cD{\dot{\bm{c}}}
%\def\dD{\dot{\bm{d}}}
%\def\eD{\dot{\bm{e}}}
%\def\fD{\dot{\bm{f}}}
%\def\gD{\dot{\bm{g}}}
%\def\hD{\dot{\bm{h}}}
%\def\iD{\dot{\bm{i}}}
%\def\iD{\dot{\bm{j}}}
%\def\kD{\dot{\bm{k}}}
%\def\lD{\dot{\bm{l}}}
%\def\mD{\dot{\bm{m}}}
%\def\nD{\dot{\bm{n}}}
%\def\oD{\dot{\bm{o}}}
%\def\pD{\dot{\bm{p}}}
%\def\qD{\dot{\bm{q}}}
%\def\rD{\dot{\bm{r}}}
%\def\sD{\dot{\bm{s}}}
%\def\tD{\dot{\bm{t}}}
%\def\uD{\dot{\bm{u}}}
%\def\vD{\dot{\bm{v}}}
%\def\wD{\dot{\bm{w}}}
\def\xD{\dot{\bm{x}}}
%\def\yD{\dot{\bm{y}}}
%\def\zD{\dot{\bm{z}}}
%\def\AD{\dot{\bm{A}}}
%\def\BD{\dot{\bm{B}}}
%\def\CD{\dot{\bm{C}}}
%\def\DD{\dot{\bm{D}}}
%\def\ED{\dot{\bm{E}}}
%\def\FD{\dot{\bm{F}}}
%\def\GD{\dot{\bm{G}}}
%\def\HD{\dot{\bm{H}}}
%\def\ID{\dot{\bm{I}}}
%\def\JD{\dot{\bm{J}}}
%\def\KD{\dot{\bm{K}}}
%\def\LD{\dot{\bm{L}}}
%\def\MD{\dot{\bm{M}}}
%\def\ND{\dot{\bm{N}}}
%\def\OD{\dot{\bm{O}}}
%\def\PD{\dot{\bm{P}}}
%\def\QD{\dot{\bm{Q}}}
%\def\RD{\dot{\bm{R}}}
%\def\SD{\dot{\bm{S}}}
%\def\TD{\dot{\bm{T}}}
%\def\UD{\dot{\bm{U}}}
%\def\VD{\dot{\bm{V}}}
%\def\WD{\dot{\bm{W}}}
%\def\XD{\dot{\bm{X}}}
%\def\YD{\dot{\bm{Y}}}
%\def\ZD{\dot{\bm{Z}}}
%
%
%% bold double dot
%\def\aDD{\ddot{\bm{a}}}
%\def\bDD{\ddot{\bm{b}}}
%\def\cDD{\ddot{\bm{c}}}
%\def\dDD{\ddot{\bm{d}}}
%\def\eDD{\ddot{\bm{e}}}
%\def\fDD{\ddot{\bm{f}}}
%\def\gDD{\ddot{\bm{g}}}
%\def\hDD{\ddot{\bm{h}}}
%\def\iDD{\ddot{\bm{i}}}
%\def\iDD{\ddot{\bm{j}}}
%\def\kDD{\ddot{\bm{k}}}
%\def\lDD{\ddot{\bm{l}}}
%\def\mDD{\ddot{\bm{m}}}
%\def\nDD{\ddot{\bm{n}}}
%\def\oDD{\ddot{\bm{o}}}
%\def\pDD{\ddot{\bm{p}}}
%\def\qDD{\ddot{\bm{q}}}
%\def\rDD{\ddot{\bm{r}}}
%\def\sDD{\ddot{\bm{s}}}
%\def\tDD{\ddot{\bm{t}}}
%\def\uDD{\ddot{\bm{u}}}
%\def\vDD{\ddot{\bm{v}}}
%\def\wDD{\ddot{\bm{w}}}
%\def\xDD{\ddot{\bm{x}}}
%\def\yDD{\ddot{\bm{y}}}
%\def\zDD{\ddot{\bm{z}}}
%\def\ADD{\ddot{\bm{A}}}
%\def\BDD{\ddot{\bm{B}}}
%\def\CDD{\ddot{\bm{C}}}
%\def\DDD{\ddot{\bm{D}}}
%\def\EDD{\ddot{\bm{E}}}
%\def\FDD{\ddot{\bm{F}}}
%\def\GDD{\ddot{\bm{G}}}
%\def\HDD{\ddot{\bm{H}}}
%\def\IDD{\ddot{\bm{I}}}
%\def\JDD{\ddot{\bm{J}}}
%\def\KDD{\ddot{\bm{K}}}
%\def\LDD{\ddot{\bm{L}}}
%\def\MDD{\ddot{\bm{M}}}
%\def\NDD{\ddot{\bm{N}}}
%\def\ODD{\ddot{\bm{O}}}
%\def\PDD{\ddot{\bm{P}}}
%\def\QDD{\ddot{\bm{Q}}}
%\def\RDD{\ddot{\bm{R}}}
%\def\SDD{\ddot{\bm{S}}}
%\def\TDD{\ddot{\bm{T}}}
%\def\UDD{\ddot{\bm{U}}}
%\def\VDD{\ddot{\bm{V}}}
%\def\WDD{\ddot{\bm{W}}}
%\def\XDD{\ddot{\bm{X}}}
%\def\YDD{\ddot{\bm{Y}}}
%\def\ZDD{\ddot{\bm{Z}}}
%
%
% hat
\def\ah{\hat{{a}}}
\def\bh{\hat{{b}}}
\def\ch{\hat{{c}}}
\def\dh{\hat{{d}}}
\def\eh{\hat{{e}}}
\def\fh{\hat{{f}}}
\def\gh{\hat{{g}}}
\def\hh{\hat{{h}}}
\def\ih{\hat{{i}}}
\def\ih{\hat{{j}}}
\def\kh{\hat{{k}}}
\def\lh{\hat{{l}}}
\def\mh{\hat{{m}}}
\def\nh{\hat{{n}}}
\def\oh{\hat{{o}}}
\def\ph{\hat{{p}}}
\def\qh{\hat{{q}}}
\def\rh{\hat{{r}}}
\def\sh{\hat{{s}}}
\def\th{\hat{{t}}}
\def\uh{\hat{{u}}}
\def\vh{\hat{{v}}}
\def\wh{\hat{{w}}}
\def\xh{\hat{{x}}}
\def\yh{\hat{{y}}}
\def\zh{\hat{{z}}}
\def\Ah{\hat{{A}}}
\def\Bh{\hat{{B}}}
\def\Ch{\hat{{C}}}
\def\Dh{\hat{{D}}}
\def\Eh{\hat{{E}}}
\def\Fh{\hat{{F}}}
\def\Gh{\hat{{G}}}
\def\Hh{\hat{{H}}}
\def\Ih{\hat{{I}}}
\def\Jh{\hat{{J}}}
\def\Kh{\hat{{K}}}
\def\Lh{\hat{{L}}}
\def\Mh{\hat{{M}}}
\def\Nh{\hat{{N}}}
\def\Oh{\hat{{O}}}
\def\Ph{\hat{{P}}}
\def\Qh{\hat{{Q}}}
\def\Rh{\hat{{R}}}
\def\Sh{\hat{{S}}}
\def\Th{\hat{{T}}}
\def\Uh{\hat{{U}}}
\def\Vh{\hat{{V}}}
\def\Wh{\hat{{W}}}
\def\Xh{\hat{{X}}}
\def\Yh{\hat{{Y}}}
\def\Zh{\hat{{Z}}}
%
% bar
\def\ab{\bar{{a}}}
\def\bb{\bar{{b}}}
\def\cb{\bar{{c}}}
\def\db{\bar{{d}}}
\def\eb{\bar{{e}}}
\def\fb{\bar{{f}}}
\def\gb{\bar{{g}}}
\def\hb{\bar{{h}}}
\def\ib{\bar{{i}}}
\def\ib{\bar{{j}}}
\def\kb{\bar{{k}}}
\def\lb{\bar{{l}}}
\def\mb{\bar{{m}}}
\def\nb{\bar{{n}}}
\def\ob{\bar{{o}}}
\def\pb{\bar{{p}}}
\def\qb{\bar{{q}}}
\def\rb{\bar{{r}}}
\def\sb{\bar{{s}}}
\def\tb{\bar{{t}}}
\def\ub{\bar{{u}}}
\def\vb{\bar{{v}}}
\def\wb{\bar{{w}}}
\def\xb{\bar{{x}}}
\def\yb{\bar{{y}}}
\def\zb{\bar{{z}}}
\def\Ab{\bar{{A}}}
\def\Bb{\bar{{B}}}
\def\Cb{\bar{{C}}}
\def\Db{\bar{{D}}}
\def\Eb{\bar{{E}}}
\def\Fb{\bar{{F}}}
\def\Gb{\bar{{G}}}
\def\Hb{\bar{{H}}}
\def\Ib{\bar{{I}}}
\def\Jb{\bar{{J}}}
\def\Kb{\bar{{K}}}
\def\Lb{\bar{{L}}}
\def\Mb{\bar{{M}}}
\def\Nb{\bar{{N}}}
\def\Ob{\bar{{O}}}
\def\Pb{\bar{{P}}}
\def\Qb{\bar{{Q}}}
\def\Rb{\bar{{R}}}
\def\Sb{\bar{{S}}}
\def\Tb{\bar{{T}}}
\def\Ub{\bar{{U}}}
\def\Vb{\bar{{V}}}
\def\Wb{\bar{{W}}}
\def\Xb{\bar{{X}}}
\def\Yb{\bar{{Y}}}
\def\Zb{\bar{{Z}}}
%
%%% tilde
%%\def\at{\tilde{{a}}}
%%\def\bt{\tilde{{b}}}
%%\def\ct{\tilde{{c}}}
%%\def\dt{\tilde{{d}}}
%%\def\et{\tilde{{e}}}
%%\def\ft{\tilde{{f}}}
%%\def\gt{\tilde{{g}}}
%%\def\htilde{\tilde{{h}}}
%%\def\it{\tilde{{i}}}
%%\def\it{\tilde{{j}}}
%%\def\kt{\tilde{{k}}}
%%\def\lt{\tilde{{l}}}
%%\def\mt{\tilde{{m}}}
%%\def\nt{\tilde{{n}}}
%%\def\ot{\tilde{{o}}}
%%\def\pt{\tilde{{p}}}
%%\def\qt{\tilde{{q}}}
%%\def\rt{\tilde{{r}}}
%%\def\st{\tilde{{s}}}
%%\def\tt{\tilde{{t}}}
%%\def\ut{\tilde{{u}}}
%%\def\vt{\tilde{{v}}}
%%\def\wt{\tilde{{w}}}
%%\def\xt{\tilde{{x}}}
%%\def\yt{\tilde{{y}}}
%%\def\zt{\tilde{{z}}}
%%\def\At{\tilde{{A}}}
%%\def\Bt{\tilde{{B}}}
%%\def\Ct{\tilde{{C}}}
%%\def\Dt{\tilde{{D}}}
%%\def\Et{\tilde{{E}}}
%%\def\Ft{\tilde{{F}}}
%%\def\Gt{\tilde{{G}}}
%%\def\Ht{\tilde{{H}}}
%%\def\It{\tilde{{I}}}
%%\def\Jt{\tilde{{J}}}
%%\def\Kt{\tilde{{K}}}
%%\def\Lt{\tilde{{L}}}
%%\def\Mt{\tilde{{M}}}
%%\def\Nt{\tilde{{N}}}
%%\def\Ot{\tilde{{O}}}
%%\def\Pt{\tilde{{P}}}
%%\def\Qt{\tilde{{Q}}}
%%\def\Rt{\tilde{{R}}}
%%\def\St{\tilde{{S}}}
%%\def\Tt{\tilde{{T}}}
%%\def\Ut{\tilde{{U}}}
%%\def\Vt{\tilde{{V}}}
%%\def\Wt{\tilde{{W}}}
%%\def\Xt{\tilde{{X}}}
%%\def\Yt{\tilde{{Y}}}
%%\def\Zt{\tilde{{Z}}}
%
%% vec
%\def\av{\vec{{a}}}
%\def\bv{\vec{{b}}}
%\def\cv{\vec{{c}}}
%\def\dv{\vec{{d}}}
%\def\ev{\vec{{e}}}
%\def\fv{\vec{{f}}}
%\def\gv{\vec{{g}}}
%\def\hv{\vec{{h}}}
%\def\iv{\vec{{i}}}
%\def\iv{\vec{{j}}}
%\def\kv{\vec{{k}}}
%\def\lv{\vec{{l}}}
%\def\mv{\vec{{m}}}
%\def\nv{\vec{{n}}}
%\def\ov{\vec{{o}}}
%\def\pv{\vec{{p}}}
%\def\qv{\vec{{q}}}
%\def\rv{\vec{{r}}}
%\def\sv{\vec{{s}}}
%\def\tv{\vec{{t}}}
%\def\uv{\vec{{u}}}
%\def\vv{\vec{{v}}}
%\def\wv{\vec{{w}}}
\def\xv{\vec{{x}}}
\def\yv{\vec{{y}}}
%\def\zv{\vec{{z}}}
%\def\Av{\vec{{A}}}
%\def\Bv{\vec{{B}}}
%\def\Cv{\vec{{C}}}
%\def\Dv{\vec{{D}}}
%\def\Ev{\vec{{E}}}
%\def\Fv{\vec{{F}}}
%\def\Gv{\vec{{G}}}
%\def\hv{\vec{{h}}}
%\def\Iv{\vec{{I}}}
%\def\Jv{\vec{{J}}}
%\def\Kv{\vec{{K}}}
%\def\Lv{\vec{{L}}}
%\def\Mv{\vec{{M}}}
%\def\Nv{\vec{{N}}}
%\def\Ov{\vec{{O}}}
%\def\Pv{\vec{{P}}}
%\def\Qv{\vec{{Q}}}
%\def\Rv{\vec{{R}}}
%\def\Sv{\vec{{S}}}
%\def\Tv{\vec{{T}}}
%\def\Uv{\vec{{U}}}
%\def\Vv{\vec{{V}}}
%\def\Wv{\vec{{W}}}
%\def\Xv{\vec{{X}}}
%\def\Yv{\vec{{Y}}}
%\def\Zv{\vec{{Z}}}
%
%% acute
%\def\aa{\acute{{a}}}
%\def\ba{\acute{{b}}}
%\def\ca{\acute{{c}}}
%\def\da{\acute{{d}}}
%\def\ea{\acute{{e}}}
%\def\fa{\acute{{f}}}
%\def\ga{\acute{{g}}}
%\def\ha{\acute{{h}}}
%\def\ia{\acute{{i}}}
%\def\ia{\acute{{j}}}
%\def\ka{\acute{{k}}}
%\def\la{\acute{{l}}}
%\def\ma{\acute{{m}}}
%\def\na{\acute{{n}}}
%\def\oa{\acute{{o}}}
%\def\pa{\acute{{p}}}
%\def\qa{\acute{{q}}}
%\def\ra{\acute{{r}}}
%\def\sa{\acute{{s}}}
%\def\ta{\acute{{t}}}
%\def\ua{\acute{{u}}}
%\def\va{\acute{{v}}}
%\def\wa{\acute{{w}}}
%\def\xa{\acute{{x}}}
%\def\ya{\acute{{y}}}
%\def\za{\acute{{z}}}
%\def\Aa{\acute{{A}}}
%\def\Ba{\acute{{B}}}
%\def\Ca{\acute{{C}}}
%\def\Da{\acute{{D}}}
%\def\Ea{\acute{{E}}}
%\def\Fa{\acute{{F}}}
%\def\Ga{\acute{{G}}}
%\def\Ha{\acute{{H}}}
%\def\Ia{\acute{{I}}}
%\def\Ja{\acute{{J}}}
%\def\Ka{\acute{{K}}}
%\def\La{\acute{{L}}}
%\def\Ma{\acute{{M}}}
%\def\Na{\acute{{N}}}
%\def\Oa{\acute{{O}}}
%\def\Pa{\acute{{P}}}
%\def\Qa{\acute{{Q}}}
%\def\Ra{\acute{{R}}}
%\def\Sa{\acute{{S}}}
%\def\Ta{\acute{{T}}}
%\def\Ua{\acute{{U}}}
%\def\Va{\acute{{V}}}
%\def\Wa{\acute{{W}}}
%\def\Xa{\acute{{X}}}
%\def\Ya{\acute{{Y}}}
%\def\Za{\acute{{Z}}}
%
%% check
%\def\ac{\check{{a}}}
%\def\bc{\check{{b}}}
%\def\cc{\check{{c}}}
%\def\dc{\check{{d}}}
%\def\ec{\check{{e}}}
%\def\fc{\check{{f}}}
%\def\gc{\check{{g}}}
%\def\hc{\check{{h}}}
%\def\ic{\check{{i}}}
%\def\ic{\check{{j}}}
%\def\kc{\check{{k}}}
%\def\lc{\check{{l}}}
%\def\mc{\check{{m}}}
%\def\nc{\check{{n}}}
%\def\oc{\check{{o}}}
%\def\pc{\check{{p}}}
%\def\qc{\check{{q}}}
%\def\rc{\check{{r}}}
%\def\sc{\check{{s}}}
%\def\tc{\check{{t}}}
%\def\uc{\check{{u}}}
%\def\vc{\check{{v}}}
%\def\wc{\check{{w}}}
%\def\xc{\check{{x}}}
%\def\yc{\check{{y}}}
%\def\zc{\check{{z}}}
%\def\Ac{\check{{A}}}
%\def\Bc{\check{{B}}}
%\def\Cc{\check{{C}}}
%\def\Dc{\check{{D}}}
%\def\Ec{\check{{E}}}
%\def\Fc{\check{{F}}}
%\def\Gc{\check{{G}}}
%\def\Hc{\check{{H}}}
%\def\Ic{\check{{I}}}
%\def\Jc{\check{{J}}}
%\def\Kc{\check{{K}}}
%\def\Lc{\check{{L}}}
%\def\Mc{\check{{M}}}
%\def\Nc{\check{{N}}}
%\def\Oc{\check{{O}}}
%\def\Pc{\check{{P}}}
%\def\Qc{\check{{Q}}}
%\def\Rc{\check{{R}}}
%\def\Sc{\check{{S}}}
%\def\Tc{\check{{T}}}
%\def\Uc{\check{{U}}}
%\def\Vc{\check{{V}}}
%\def\Wc{\check{{W}}}
%\def\Xc{\check{{X}}}
%\def\Yc{\check{{Y}}}
%\def\Zc{\check{{Z}}}
%
%
%% dot
\def\ad{\dot{{a}}}
\def\bd{\dot{{b}}}
\def\cd{\dot{{c}}}
\def\dd{\dot{{d}}}
\def\ed{\dot{{e}}}
\def\fd{\dot{{f}}}
\def\gd{\dot{{g}}}
\def\hd{\dot{{h}}}
\def\id{\dot{{i}}}
\def\id{\dot{{j}}}
\def\kd{\dot{{k}}}
\def\ld{\dot{{l}}}
\def\md{\dot{{m}}}
\def\nd{\dot{{n}}}
\def\od{\dot{{o}}}
\def\pd{\dot{{p}}}
\def\qd{\dot{{q}}}
\def\rd{\dot{{r}}}
\def\sd{\dot{{s}}}
\def\td{\dot{{t}}}
\def\ud{\dot{{u}}}
\def\vd{\dot{{v}}}
\def\wdot{\dot{{w}}}
\def\xd{\dot{{x}}}
\def\yd{\dot{{y}}}
\def\zd{\dot{{z}}}
\def\Ad{\dot{{A}}}
\def\Bd{\dot{{B}}}
\def\Cd{\dot{{C}}}
\def\Dd{\dot{{D}}}
\def\Ed{\dot{{E}}}
\def\Fd{\dot{{F}}}
\def\Gd{\dot{{G}}}
\def\Hd{\dot{{H}}}
\def\Id{\dot{{I}}}
\def\Jd{\dot{{J}}}
\def\Kd{\dot{{K}}}
\def\Ld{\dot{{L}}}
\def\Md{\dot{{M}}}
\def\Nd{\dot{{N}}}
\def\Od{\dot{{O}}}
\def\Pd{\dot{{P}}}
\def\Qd{\dot{{Q}}}
\def\Rd{\dot{{R}}}
\def\Sd{\dot{{S}}}
\def\Td{\dot{{T}}}
\def\Ud{\dot{{U}}}
\def\Vd{\dot{{V}}}
\def\Wd{\dot{{W}}}
\def\Xd{\dot{{X}}}
\def\Yd{\dot{{Y}}}
\def\Zd{\dot{{Z}}}
%
%
%% double dot
%\def\add{\ddot{{a}}}
%\def\bdd{\ddot{{b}}}
%\def\cdd{\ddot{{c}}}
%\def\ddd{\ddot{{d}}}
%\def\edd{\ddot{{e}}}
%\def\fdd{\ddot{{f}}}
%\def\gdd{\ddot{{g}}}
%\def\hdd{\ddot{{h}}}
%\def\idd{\ddot{{i}}}
%\def\idd{\ddot{{j}}}
%\def\kdd{\ddot{{k}}}
%\def\ldd{\ddot{{l}}}
%\def\mdd{\ddot{{m}}}
%\def\ndd{\ddot{{n}}}
%\def\odd{\ddot{{o}}}
%\def\pdd{\ddot{{p}}}
%\def\qdd{\ddot{{q}}}
%\def\rdd{\ddot{{r}}}
%\def\sdd{\ddot{{s}}}
%\def\tdd{\ddot{{t}}}
%\def\udd{\ddot{{u}}}
%\def\vdd{\ddot{{v}}}
%\def\wdd{\ddot{{w}}}
%\def\xdd{\ddot{{x}}}
%\def\ydd{\ddot{{y}}}
%\def\zdd{\ddot{{z}}}
%\def\Add{\ddot{{A}}}
%\def\Bdd{\ddot{{B}}}
%\def\Cdd{\ddot{{C}}}
%\def\Ddd{\ddot{{D}}}
%\def\Edd{\ddot{{E}}}
%\def\Fdd{\ddot{{F}}}
%\def\Gdd{\ddot{{G}}}
%\def\Hdd{\ddot{{H}}}
%\def\Idd{\ddot{{I}}}
%\def\Jdd{\ddot{{J}}}
%\def\Kdd{\ddot{{K}}}
%\def\Ldd{\ddot{{L}}}
%\def\Mdd{\ddot{{M}}}
%\def\Ndd{\ddot{{N}}}
%\def\Odd{\ddot{{O}}}
%\def\Pdd{\ddot{{P}}}
%\def\Qdd{\ddot{{Q}}}
%\def\Rdd{\ddot{{R}}}
%\def\Sdd{\ddot{{S}}}
%\def\Tdd{\ddot{{T}}}
%\def\Udd{\ddot{{U}}}
%\def\Vdd{\ddot{{V}}}
%\def\Wdd{\ddot{{W}}}
%\def\Xdd{\ddot{{X}}}
%\def\Ydd{\ddot{{Y}}}
%\def\Zdd{\ddot{{Z}}}
%
%
%% script 
\def\as{\mathcal{{a}}}
\def\bs{\mathcal{{b}}}
\def\cs{\mathcal{{c}}}
\def\ds{\mathcal{{d}}}
\def\es{\mathcal{{e}}}
\def\fs{\mathcal{{f}}}
\def\gs{\mathcal{{g}}}
\def\hs{\mathcal{{h}}}
\def\is{\mathcal{{i}}}
\def\is{\mathcal{{j}}}
\def\ks{\mathcal{{k}}}
\def\ls{\mathcal{{l}}}
\def\ms{\mathcal{{m}}}
\def\ns{\mathcal{{n}}}
\def\os{\mathcal{{o}}}
\def\ps{\mathcal{{p}}}
\def\qs{\mathcal{{q}}}
\def\rs{\mathcal{{r}}}
\def\ss{\mathcal{{s}}}
\def\ts{\mathcal{{t}}}
\def\us{\mathcal{{u}}}
\def\vs{\mathcal{{v}}}
\def\ws{\mathcal{{w}}}
\def\xs{\mathcal{{x}}}
\def\ys{\mathcal{{y}}}
\def\zs{\mathcal{{z}}}
\def\As{\mathcal{{A}}}
\def\Bs{\mathcal{{B}}}
\def\Cs{\mathcal{{C}}}
\def\Ds{\mathcal{{D}}}
\def\Es{\mathcal{{E}}}
\def\Fs{\mathcal{{F}}}
\def\Gs{\mathcal{{G}}}
\def\Gsh{\hat{\mathcal{{G}}}}
\def\Hs{\mathcal{{H}}}
\def\Hsh{\hat{\mathcal{{H}}}}
\def\Is{\mathcal{{I}}}
\def\Js{\mathcal{{J}}}
\def\Ks{\mathcal{{K}}}
\def\Ksh{\hat{\mathcal{{K}}}}
\def\Ksb{\bar{\mathcal{{K}}}}
\def\Ls{\mathcal{{L}}}
\def\Ms{\mathcal{{M}}}
\def\Ns{\mathcal{{N}}}
\def\Os{\mathcal{{O}}}
\def\Ps{\mathcal{{P}}}
\def\Qs{\mathcal{{Q}}}
\def\Rs{\mathcal{{R}}}
\def\Ss{\mathcal{{S}}}
\def\Ts{\mathcal{{T}}}
\def\Us{\mathcal{{U}}}
\def\Vs{\mathcal{{V}}}
\def\Ws{\mathcal{{W}}}
\def\Xs{\mathcal{{X}}}
\def\Ys{\mathcal{{Y}}}
\def\Ysh{\widehat{\mathcal{Y}}}
\def\Zs{\mathcal{{Z}}}
%
%% bold greeks
\def\alphaB{{\bm{\alpha}}}
\def\betaB{{\bm{\beta}}}
\def\gammaB{{\bm{\gamma}}}
\def\deltaB{{\bm{\delta}}}
\def\epsilonB{{\bm{\epsilon}}}
\def\zetaB{{\bm{\zeta}}}
\def\etaB{{\bm{\eta}}}
\def\thetaB{{\bm{\theta}}}
\def\iotaB{{\bm{\iota}}}
\def\kappaB{{\bm{\kappa}}}
\def\lambdaB{{\bm{\lambda}}}
\def\muB{{\bm{\mu}}}
\def\nuB{{\bm{\nu}}}
\def\piB{{\bm{\pi}}}
\def\rhoB{{\bm{\rho}}}
\def\sigmaB{{\bm{\sigma}}}
\def\tauB{{\bm{\tau}}}
\def\upsilonB{{\bm{\upsilon}}}
\def\phiB{{\bm{\phi}}}
\def\chiB{{\bm{\chi}}}
\def\psiB{{\bm{\psi}}}
\def\omegaB{{\bm{\omega}}}
\def\GammaB{{\bm{\Gamma}}}
\def\DeltaB{{\bm{\Delta}}}
\def\ThetaB{{\bm{\Theta}}}
\def\LambdaB{{\bm{\Lambda}}}
\def\PiB{{\bm{\Pi}}}
\def\SigmaB{{\bm{\Sigma}}}
\def\UpsilonB{{\bm{\Upsilon}}}
\def\PhiB{{\bm{\Phi}}}
\def\PsiB{{\bm{\Psi}}}
\def\OmegaB{{\bm{\Omega}}}
%
%
%% bold hat greeks
%\def\alphaBH{\hat{\bm{\alpha}}}
%\def\betaBH{\hat{\bm{\beta}}}
\def\gammaBH{\hat{\bm{\gamma}}}
%\def\deltaBH{\hat{\bm{\delta}}}
%\def\epsilonBH{\hat{\bm{\epsilon}}}
%\def\zetaBH{\hat{\bm{\zeta}}}
%\def\etaBH{\hat{\bm{\eta}}}
\def\thetaBH{\hat{\bm{\theta}}}
%\def\iotaBH{\hat{\bm{\iota}}}
%\def\kappaBH{\hat{\bm{\kappa}}}
%\def\lambdaBH{\hat{\bm{\lambda}}}
\def\muBH{\hat{\bm{\mu}}}
%\def\nuBH{\hat{\bm{\nu}}}
%\def\piBH{\hat{\bm{\pi}}}
\def\rhoBH{\hat{\bm{\rho}}}
%\def\sigmaBH{\hat{\bm{\sigma}}}
%\def\tauBH{\hat{\bm{\tau}}}
%\def\upsilonBH{\hat{\bm{\upsilon}}}
%\def\phiBH{\hat{\bm{\phi}}}
%\def\chiBH{\hat{\bm{\chi}}}
%\def\psiBH{\hat{\bm{\psi}}}
%\def\omegaBH{\hat{\bm{\omega}}}
%\def\GammaBH{\hat{\bm{\Gamma}}}
%\def\DeltaBH{\hat{\bm{\Delta}}}
%\def\ThetaBH{\hat{\bm{\Theta}}}
%\def\LambdaBH{\hat{\bm{\Lambda}}}
%\def\PiBH{\hat{\bm{\Pi}}}
%\def\SigmaBH{\hat{\bm{\Sigma}}}
%\def\UpsilonBH{\hat{\bm{\Upsilon}}}
%\def\PhiBH{\hat{\bm{\Phi}}}
%\def\PsiBH{\hat{\bm{\Psi}}}
%\def\OmegaBH{\hat{\bm{\Omega}}}
%
%
%% bold bar greeks
%\def\alphaBB{\bar{\bm{\alpha}}}
%\def\betaBB{\bar{\bm{\beta}}}
%\def\gammaBB{\bar{\bm{\gamma}}}
%\def\deltaBB{\bar{\bm{\delta}}}
%\def\epsilonBB{\bar{\bm{\epsilon}}}
%\def\zetaBB{\bar{\bm{\zeta}}}
%\def\etaBB{\bar{\bm{\eta}}}
\def\thetaBB{\bar{\bm{\theta}}}
%\def\iotaBB{\bar{\bm{\iota}}}
%\def\kappaBB{\bar{\bm{\kappa}}}
%\def\lambdaBB{\bar{\bm{\lambda}}}
\def\muBB{\bar{\bm{\mu}}}
%\def\nuBB{\bar{\bm{\nu}}}
%\def\piBB{\bar{\bm{\pi}}}
\def\rhoBB{\bar{\bm{\rho}}}
%\def\sigmaBB{\bar{\bm{\sigma}}}
%\def\tauBB{\bar{\bm{\tau}}}
%\def\upsilonBB{\bar{\bm{\upsilon}}}
%\def\phiBB{\bar{\bm{\phi}}}
%\def\chiBB{\bar{\bm{\chi}}}
%\def\psiBB{\bar{\bm{\psi}}}
%\def\omegaBB{\bar{\bm{\omega}}}
%\def\GammaBB{\bar{\bm{\Gamma}}}
%\def\DeltaBB{\bar{\bm{\Delta}}}
%\def\ThetaBB{\bar{\bm{\Theta}}}
%\def\LambdaBB{\bar{\bm{\Lambda}}}
%\def\PiBB{\bar{\bm{\Pi}}}
%\def\SigmaBB{\bar{\bm{\Sigma}}}
%\def\UpsilonBB{\bar{\bm{\Upsilon}}}
%\def\PhiBB{\bar{\bm{\Phi}}}
%\def\PsiBB{\bar{\bm{\Psi}}}
%\def\OmegaBB{\bar{\bm{\Omega}}}
%
%% bold tilde greeks
%\def\alphaBT{\tilde{\bm{\alpha}}}
%\def\betaBT{\tilde{\bm{\beta}}}
%\def\gammaBT{\tilde{\bm{\gamma}}}
%\def\deltaBT{\tilde{\bm{\delta}}}
%\def\epsilonBT{\tilde{\bm{\epsilon}}}
%\def\zetaBT{\tilde{\bm{\zeta}}}
%\def\etaBT{\tilde{\bm{\eta}}}
%\def\thetaBT{\tilde{\bm{\theta}}}
%\def\iotaBT{\tilde{\bm{\iota}}}
%\def\kappaBT{\tilde{\bm{\kappa}}}
%\def\lambdaBT{\tilde{\bm{\lambda}}}
%\def\muBT{\tilde{\bm{\mu}}}
%\def\nuBT{\tilde{\bm{\nu}}}
%\def\piBT{\tilde{\bm{\pi}}}
%\def\rhoBT{\tilde{\bm{\rho}}}
%\def\sigmaBT{\tilde{\bm{\sigma}}}
%\def\tauBT{\tilde{\bm{\tau}}}
%\def\upsilonBT{\tilde{\bm{\upsilon}}}
%\def\phiBT{\tilde{\bm{\phi}}}
%\def\chiBT{\tilde{\bm{\chi}}}
%\def\psiBT{\tilde{\bm{\psi}}}
%\def\omegaBT{\tilde{\bm{\omega}}}
%\def\GammaBT{\tilde{\bm{\Gamma}}}
%\def\DeltaBT{\tilde{\bm{\Delta}}}
%\def\ThetaBT{\tilde{\bm{\Theta}}}
%\def\LambdaBT{\tilde{\bm{\Lambda}}}
%\def\PiBT{\tilde{\bm{\Pi}}}
%\def\SigmaBT{\tilde{\bm{\Sigma}}}
%\def\UpsilonBT{\tilde{\bm{\Upsilon}}}
%\def\PhiBT{\tilde{\bm{\Phi}}}
%\def\PsiBT{\tilde{\bm{\Psi}}}
%\def\OmegaBT{\tilde{\bm{\Omega}}}
%
%
%% bold vec greeks
%\def\alphaBV{\vec{\bm{\alpha}}}
%\def\betaBV{\vec{\bm{\beta}}}
%\def\gammaBV{\vec{\bm{\gamma}}}
%\def\deltaBV{\vec{\bm{\delta}}}
%\def\epsilonBV{\vec{\bm{\epsilon}}}
%\def\zetaBV{\vec{\bm{\zeta}}}
%\def\etaBV{\vec{\bm{\eta}}}
%\def\thetaBV{\vec{\bm{\theta}}}
%\def\iotaBV{\vec{\bm{\iota}}}
%\def\kappaBV{\vec{\bm{\kappa}}}
%\def\lambdaBV{\vec{\bm{\lambda}}}
%\def\muBV{\vec{\bm{\mu}}}
%\def\nuBV{\vec{\bm{\nu}}}
%\def\piBV{\vec{\bm{\pi}}}
%\def\rhoBV{\vec{\bm{\rho}}}
%\def\sigmaBV{\vec{\bm{\sigma}}}
%\def\tauBV{\vec{\bm{\tau}}}
%\def\upsilonBV{\vec{\bm{\upsilon}}}
%\def\phiBV{\vec{\bm{\phi}}}
%\def\chiBV{\vec{\bm{\chi}}}
%\def\psiBV{\vec{\bm{\psi}}}
%\def\omegaBV{\vec{\bm{\omega}}}
%\def\GammaBV{\vec{\bm{\Gamma}}}
%\def\DeltaBV{\vec{\bm{\Delta}}}
%\def\ThetaBV{\vec{\bm{\Theta}}}
%\def\LambdaBV{\vec{\bm{\Lambda}}}
%\def\PiBV{\vec{\bm{\Pi}}}
%\def\SigmaBV{\vec{\bm{\Sigma}}}
%\def\UpsilonBV{\vec{\bm{\Upsilon}}}
%\def\PhiBV{\vec{\bm{\Phi}}}
%\def\PsiBV{\vec{\bm{\Psi}}}
%\def\OmegaBV{\vec{\bm{\Omega}}}
%
%% bold acute greeks
%\def\alphaBA{\acute{\bm{\alpha}}}
%\def\betaBA{\acute{\bm{\beta}}}
%\def\gammaBA{\acute{\bm{\gamma}}}
%\def\deltaBA{\acute{\bm{\delta}}}
%\def\epsilonBA{\acute{\bm{\epsilon}}}
%\def\zetaBA{\acute{\bm{\zeta}}}
%\def\etaBA{\acute{\bm{\eta}}}
%\def\thetaBA{\acute{\bm{\theta}}}
%\def\iotaBA{\acute{\bm{\iota}}}
%\def\kappaBA{\acute{\bm{\kappa}}}
%\def\lambdaBA{\acute{\bm{\lambda}}}
%\def\muBA{\acute{\bm{\mu}}}
%\def\nuBA{\acute{\bm{\nu}}}
%\def\piBA{\acute{\bm{\pi}}}
%\def\rhoBA{\acute{\bm{\rho}}}
%\def\sigmaBA{\acute{\bm{\sigma}}}
%\def\tauBA{\acute{\bm{\tau}}}
%\def\upsilonBA{\acute{\bm{\upsilon}}}
%\def\phiBA{\acute{\bm{\phi}}}
%\def\chiBA{\acute{\bm{\chi}}}
%\def\psiBA{\acute{\bm{\psi}}}
%\def\omegaBA{\acute{\bm{\omega}}}
%\def\GammaBA{\acute{\bm{\Gamma}}}
%\def\DeltaBA{\acute{\bm{\Delta}}}
%\def\ThetaBA{\acute{\bm{\Theta}}}
%\def\LambdaBA{\acute{\bm{\Lambda}}}
%\def\PiBA{\acute{\bm{\Pi}}}
%\def\SigmaBA{\acute{\bm{\Sigma}}}
%\def\UpsilonBA{\acute{\bm{\Upsilon}}}
%\def\PhiBA{\acute{\bm{\Phi}}}
%\def\PsiBA{\acute{\bm{\Psi}}}
%\def\OmegaBA{\acute{\bm{\Omega}}}
%
%
%% bold check greeks
%\def\alphaBC{\check{\bm{\alpha}}}
%\def\betaBC{\check{\bm{\beta}}}
%\def\gammaBC{\check{\bm{\gamma}}}
%\def\deltaBC{\check{\bm{\delta}}}
%\def\epsilonBC{\check{\bm{\epsilon}}}
%\def\zetaBC{\check{\bm{\zeta}}}
%\def\etaBC{\check{\bm{\eta}}}
%\def\thetaBC{\check{\bm{\theta}}}
%\def\iotaBC{\check{\bm{\iota}}}
%\def\kappaBC{\check{\bm{\kappa}}}
%\def\lambdaBC{\check{\bm{\lambda}}}
%\def\muBC{\check{\bm{\mu}}}
%\def\nuBC{\check{\bm{\nu}}}
%\def\piBC{\check{\bm{\pi}}}
%\def\rhoBC{\check{\bm{\rho}}}
%\def\sigmaBC{\check{\bm{\sigma}}}
%\def\tauBC{\check{\bm{\tau}}}
%\def\upsilonBC{\check{\bm{\upsilon}}}
%\def\phiBC{\check{\bm{\phi}}}
%\def\chiBC{\check{\bm{\chi}}}
%\def\psiBC{\check{\bm{\psi}}}
%\def\omegaBC{\check{\bm{\omega}}}
%\def\GammaBC{\check{\bm{\Gamma}}}
%\def\DeltaBC{\check{\bm{\Delta}}}
%\def\ThetaBC{\check{\bm{\Theta}}}
%\def\LambdaBC{\check{\bm{\Lambda}}}
%\def\PiBC{\check{\bm{\Pi}}}
%\def\SigmaBC{\check{\bm{\Sigma}}}
%\def\UpsilonBC{\check{\bm{\Upsilon}}}
%\def\PhiBC{\check{\bm{\Phi}}}
%\def\PsiBC{\check{\bm{\Psi}}}
%\def\OmegaBC{\check{\bm{\Omega}}}
%
%
%% bold dot greeks
%\def\alphaBD{\dot{\bm{\alpha}}}
%\def\betaBD{\dot{\bm{\beta}}}
%\def\gammaBD{\dot{\bm{\gamma}}}
%\def\deltaBD{\dot{\bm{\delta}}}
%\def\epsilonBD{\dot{\bm{\epsilon}}}
%\def\zetaBD{\dot{\bm{\zeta}}}
%\def\etaBD{\dot{\bm{\eta}}}
%\def\thetaBD{\dot{\bm{\theta}}}
%\def\iotaBD{\dot{\bm{\iota}}}
%\def\kappaBD{\dot{\bm{\kappa}}}
%\def\lambdaBD{\dot{\bm{\lambda}}}
%\def\muBD{\dot{\bm{\mu}}}
%\def\nuBD{\dot{\bm{\nu}}}
%\def\piBD{\dot{\bm{\pi}}}
%\def\rhoBD{\dot{\bm{\rho}}}
%\def\sigmaBD{\dot{\bm{\sigma}}}
%\def\tauBD{\dot{\bm{\tau}}}
%\def\upsilonBD{\dot{\bm{\upsilon}}}
%\def\phiBD{\dot{\bm{\phi}}}
%\def\chiBD{\dot{\bm{\chi}}}
%\def\psiBD{\dot{\bm{\psi}}}
%\def\omegaBD{\dot{\bm{\omega}}}
%\def\GammaBD{\dot{\bm{\Gamma}}}
%\def\DeltaBD{\dot{\bm{\Delta}}}
%\def\ThetaBD{\dot{\bm{\Theta}}}
%\def\LambdaBD{\dot{\bm{\Lambda}}}
%\def\PiBD{\dot{\bm{\Pi}}}
%\def\SigmaBD{\dot{\bm{\Sigma}}}
%\def\UpsilonBD{\dot{\bm{\Upsilon}}}
%\def\PhiBD{\dot{\bm{\Phi}}}
%\def\PsiBD{\dot{\bm{\Psi}}}
%\def\OmegaBD{\dot{\bm{\Omega}}}
%
%
%% bold double dot greeks
%\def\alphaBDD{\ddot{\bm{\alpha}}}
%\def\betaBDD{\ddot{\bm{\beta}}}
%\def\gammaBDD{\ddot{\bm{\gamma}}}
%\def\deltaBDD{\ddot{\bm{\delta}}}
%\def\epsilonBDD{\ddot{\bm{\epsilon}}}
%\def\zetaBDD{\ddot{\bm{\zeta}}}
%\def\etaBDD{\ddot{\bm{\eta}}}
%\def\thetaBDD{\ddot{\bm{\theta}}}
%\def\iotaBDD{\ddot{\bm{\iota}}}
%\def\kappaBDD{\ddot{\bm{\kappa}}}
%\def\lambdaBDD{\ddot{\bm{\lambda}}}
%\def\muBDD{\ddot{\bm{\mu}}}
%\def\nuBDD{\ddot{\bm{\nu}}}
%\def\piBDD{\ddot{\bm{\pi}}}
%\def\rhoBDD{\ddot{\bm{\rho}}}
%\def\sigmaBDD{\ddot{\bm{\sigma}}}
%\def\tauBDD{\ddot{\bm{\tau}}}
%\def\upsilonBDD{\ddot{\bm{\upsilon}}}
%\def\phiBDD{\ddot{\bm{\phi}}}
%\def\chiBDD{\ddot{\bm{\chi}}}
%\def\psiBDD{\ddot{\bm{\psi}}}
%\def\omegaBDD{\ddot{\bm{\omega}}}
%\def\GammaBDD{\ddot{\bm{\Gamma}}}
%\def\DeltaBDD{\ddot{\bm{\Delta}}}
%\def\ThetaBDD{\ddot{\bm{\Theta}}}
%\def\LambdaBDD{\ddot{\bm{\Lambda}}}
%\def\PiBDD{\ddot{\bm{\Pi}}}
%\def\SigmaBDD{\ddot{\bm{\Sigma}}}
%\def\UpsilonBDD{\ddot{\bm{\Upsilon}}}
%\def\PhiBDD{\ddot{\bm{\Phi}}}
%\def\PsiBDD{\ddot{\bm{\Psi}}}
%\def\OmegaBDD{\ddot{\bm{\Omega}}}
%
%
%
%%  hat greeks
\def\alphah{\hat{{\alpha}}}
\def\betah{\hat{{\beta}}}
\def\gammah{\hat{{\gamma}}}
\def\deltah{\hat{{\delta}}}
\def\epsilonh{\hat{{\epsilon}}}
\def\zetah{\hat{{\zeta}}}
\def\etah{\hat{{\eta}}}
\def\thetah{\hat{{\theta}}}
\def\iotah{\hat{{\iota}}}
\def\kappah{\hat{{\kappa}}}
\def\lambdah{\hat{{\lambda}}}
\def\muh{\hat{{\mu}}}
\def\nuh{\hat{{\nu}}}
\def\pih{\hat{{\pi}}}
\def\rhoh{\hat{{\rho}}}
\def\sigmah{\hat{{\sigma}}}
\def\tauh{\hat{{\tau}}}
\def\upsilonh{\hat{{\upsilon}}}
\def\phih{\hat{{\phi}}}
\def\chih{\hat{{\chi}}}
\def\psih{\hat{{\psi}}}
\def\omegah{\hat{{\omega}}}
\def\Gammah{\hat{{\Gamma}}}
\def\Deltah{\hat{{\Delta}}}
\def\Thetah{\hat{{\Theta}}}
\def\Lambdah{\hat{{\Lambda}}}
\def\Pih{\hat{{\Pi}}}
\def\Sigmah{\hat{{\Sigma}}}
\def\Upsilonh{\hat{{\Upsilon}}}
\def\Phih{\hat{{\Phi}}}
\def\Psih{\hat{{\Psi}}}
\def\Omegah{\hat{{\Omega}}}
%
%
%%  bar greeks
%\def\alphab{\bar{{\alpha}}}
%\def\betab{\bar{{\beta}}}
%\def\gammab{\bar{{\gamma}}}
%\def\deltab{\bar{{\delta}}}
%\def\epsilonb{\bar{{\epsilon}}}
%\def\zetab{\bar{{\zeta}}}
%\def\etab{\bar{{\eta}}}
\def\thetab{\bar{{\theta}}}
%\def\iotab{\bar{{\iota}}}
%\def\kappab{\bar{{\kappa}}}
%\def\lambdab{\bar{{\lambda}}}
%\def\mub{\bar{{\mu}}}
%\def\nub{\bar{{\nu}}}
%\def\pib{\bar{{\pi}}}
%\def\rhob{\bar{{\rho}}}
\def\sigmab{\bar{{\sigma}}}
%\def\taub{\bar{{\tau}}}
%\def\upsilonb{\bar{{\upsilon}}}
%\def\phib{\bar{{\phi}}}
%\def\chib{\bar{{\chi}}}
%\def\psib{\bar{{\psi}}}
%\def\omegab{\bar{{\omega}}}
%\def\Gammab{\bar{{\Gamma}}}
%\def\Deltab{\bar{{\Delta}}}
%\def\Thetab{\bar{{\Theta}}}
%\def\Lambdab{\bar{{\Lambda}}}
%\def\Pib{\bar{{\Pi}}}
%\def\Sigmab{\bar{{\Sigma}}}
%\def\Upsilonb{\bar{{\Upsilon}}}
%\def\Phib{\bar{{\Phi}}}
%\def\Psib{\bar{{\Psi}}}
%\def\Omegab{\bar{{\Omega}}}
%
%%  tilde greeks
%\def\alphat{\tilde{{\alpha}}}
%\def\betat{\tilde{{\beta}}}
%\def\gammat{\tilde{{\gamma}}}
%\def\deltat{\tilde{{\delta}}}
%\def\epsilont{\tilde{{\epsilon}}}
%\def\zetat{\tilde{{\zeta}}}
%\def\etat{\tilde{{\eta}}}
%\def\thetat{\tilde{{\theta}}}
%\def\iotat{\tilde{{\iota}}}
%\def\kappat{\tilde{{\kappa}}}
%\def\lambdat{\tilde{{\lambda}}}
%\def\mut{\tilde{{\mu}}}
%\def\nut{\tilde{{\nu}}}
%\def\pit{\tilde{{\pi}}}
%\def\rhot{\tilde{{\rho}}}
%\def\sigmat{\tilde{{\sigma}}}
%\def\taut{\tilde{{\tau}}}
%\def\upsilont{\tilde{{\upsilon}}}
%\def\phit{\tilde{{\phi}}}
%\def\chit{\tilde{{\chi}}}
%\def\psit{\tilde{{\psi}}}
%\def\omegat{\tilde{{\omega}}}
%\def\Gammat{\tilde{{\Gamma}}}
%\def\Deltat{\tilde{{\Delta}}}
%\def\Thetat{\tilde{{\Theta}}}
%\def\Lambdat{\tilde{{\Lambda}}}
%\def\Pit{\tilde{{\Pi}}}
%\def\Sigmat{\tilde{{\Sigma}}}
%\def\Upsilont{\tilde{{\Upsilon}}}
%\def\Phit{\tilde{{\Phi}}}
%\def\Psit{\tilde{{\Psi}}}
%\def\Omegat{\tilde{{\Omega}}}
%
%
%%  vec greeks
%\def\alphav{\vec{{\alpha}}}
%\def\betav{\vec{{\beta}}}
%\def\gammav{\vec{{\gamma}}}
%\def\deltav{\vec{{\delta}}}
%\def\epsilonv{\vec{{\epsilon}}}
%\def\zetav{\vec{{\zeta}}}
%\def\etav{\vec{{\eta}}}
%\def\thetav{\vec{{\theta}}}
%\def\iotav{\vec{{\iota}}}
%\def\kappav{\vec{{\kappa}}}
%\def\lambdav{\vec{{\lambda}}}
%\def\muv{\vec{{\mu}}}
%\def\nuv{\vec{{\nu}}}
%\def\piv{\vec{{\pi}}}
%\def\rhov{\vec{{\rho}}}
%\def\sigmav{\vec{{\sigma}}}
%\def\tauv{\vec{{\tau}}}
%\def\upsilonv{\vec{{\upsilon}}}
%\def\phiv{\vec{{\phi}}}
%\def\chiv{\vec{{\chi}}}
%\def\psiv{\vec{{\psi}}}
%\def\omegav{\vec{{\omega}}}
%\def\Gammav{\vec{{\Gamma}}}
%\def\Deltav{\vec{{\Delta}}}
%\def\Thetav{\vec{{\Theta}}}
%\def\Lambdav{\vec{{\Lambda}}}
%\def\Piv{\vec{{\Pi}}}
%\def\Sigmav{\vec{{\Sigma}}}
%\def\Upsilonv{\vec{{\Upsilon}}}
%\def\Phiv{\vec{{\Phi}}}
%\def\Psiv{\vec{{\Psi}}}
%\def\Omegav{\vec{{\Omega}}}
%
%%  acute greeks
%\def\alphaa{\acute{{\alpha}}}
%\def\betaa{\acute{{\beta}}}
%\def\gammaa{\acute{{\gamma}}}
%\def\deltaa{\acute{{\delta}}}
%\def\epsilona{\acute{{\epsilon}}}
%\def\zetaa{\acute{{\zeta}}}
%\def\etaa{\acute{{\eta}}}
%\def\thetaa{\acute{{\theta}}}
%\def\iotaa{\acute{{\iota}}}
%\def\kappaa{\acute{{\kappa}}}
%\def\lambdaa{\acute{{\lambda}}}
%\def\mua{\acute{{\mu}}}
%\def\nua{\acute{{\nu}}}
%\def\pia{\acute{{\pi}}}
%\def\rhoa{\acute{{\rho}}}
%\def\sigmaa{\acute{{\sigma}}}
%\def\taua{\acute{{\tau}}}
%\def\upsilona{\acute{{\upsilon}}}
%\def\phia{\acute{{\phi}}}
%\def\chia{\acute{{\chi}}}
%\def\psia{\acute{{\psi}}}
%\def\omegaa{\acute{{\omega}}}
%\def\Gammaa{\acute{{\Gamma}}}
%\def\Deltaa{\acute{{\Delta}}}
%\def\Thetaa{\acute{{\Theta}}}
%\def\Lambdaa{\acute{{\Lambda}}}
%\def\Pia{\acute{{\Pi}}}
%\def\Sigmaa{\acute{{\Sigma}}}
%\def\Upsilona{\acute{{\Upsilon}}}
%\def\Phia{\acute{{\Phi}}}
%\def\Psia{\acute{{\Psi}}}
%\def\Omegaa{\acute{{\Omega}}}
%
%
%%  check greeks
%\def\alphac{\check{{\alpha}}}
%\def\betac{\check{{\beta}}}
%\def\gammac{\check{{\gamma}}}
%\def\deltac{\check{{\delta}}}
%\def\epsilonc{\check{{\epsilon}}}
%\def\zetac{\check{{\zeta}}}
%\def\etac{\check{{\eta}}}
%\def\thetac{\check{{\theta}}}
%\def\iotac{\check{{\iota}}}
%\def\kappac{\check{{\kappa}}}
%\def\lambdac{\check{{\lambda}}}
%\def\muc{\check{{\mu}}}
%\def\nuc{\check{{\nu}}}
%\def\pic{\check{{\pi}}}
%\def\rhoc{\check{{\rho}}}
%\def\sigmac{\check{{\sigma}}}
%\def\tauc{\check{{\tau}}}
%\def\upsilonc{\check{{\upsilon}}}
%\def\phic{\check{{\phi}}}
%\def\chic{\check{{\chi}}}
%\def\psic{\check{{\psi}}}
%\def\omegac{\check{{\omega}}}
%\def\Gammac{\check{{\Gamma}}}
%\def\Deltac{\check{{\Delta}}}
%\def\Thetac{\check{{\Theta}}}
%\def\Lambdac{\check{{\Lambda}}}
%\def\Pic{\check{{\Pi}}}
%\def\Sigmac{\check{{\Sigma}}}
%\def\Upsilonc{\check{{\Upsilon}}}
%\def\Phic{\check{{\Phi}}}
%\def\Psic{\check{{\Psi}}}
%\def\Omegac{\check{{\Omega}}}
%
%
%
%%  dot greeks
%\def\alphad{\dot{{\alpha}}}
%\def\betad{\dot{{\beta}}}
%\def\gammad{\dot{{\gamma}}}
%\def\deltad{\dot{{\delta}}}
%\def\epsilond{\dot{{\epsilon}}}
%\def\zetad{\dot{{\zeta}}}
%\def\etad{\dot{{\eta}}}
%\def\thetad{\dot{{\theta}}}
%\def\iotad{\dot{{\iota}}}
%\def\kappad{\dot{{\kappa}}}
%\def\lambdad{\dot{{\lambda}}}
%\def\mud{\dot{{\mu}}}
%\def\nud{\dot{{\nu}}}
%\def\pid{\dot{{\pi}}}
%\def\rhod{\dot{{\rho}}}
%\def\sigmad{\dot{{\sigma}}}
%\def\taud{\dot{{\tau}}}
%\def\upsilond{\dot{{\upsilon}}}
%\def\phid{\dot{{\phi}}}
%\def\chid{\dot{{\chi}}}
%\def\psid{\dot{{\psi}}}
%\def\omegad{\dot{{\omega}}}
%\def\Gammad{\dot{{\Gamma}}}
%\def\Deltad{\dot{{\Delta}}}
%\def\Thetad{\dot{{\Theta}}}
%\def\Lambdad{\dot{{\Lambda}}}
%\def\Pid{\dot{{\Pi}}}
%\def\Sigmad{\dot{{\Sigma}}}
%\def\Upsilond{\dot{{\Upsilon}}}
%\def\Phid{\dot{{\Phi}}}
%\def\Psid{\dot{{\Psi}}}
%\def\Omegad{\dot{{\Omega}}}
%
%
%%  double dot greeks
%\def\alphadd{\ddot{{\alpha}}}
%\def\betadd{\ddot{{\beta}}}
%\def\gammadd{\ddot{{\gamma}}}
%\def\deltadd{\ddot{{\delta}}}
%\def\epsilondd{\ddot{{\epsilon}}}
%\def\zetadd{\ddot{{\zeta}}}
%\def\etadd{\ddot{{\eta}}}
%\def\thetadd{\ddot{{\theta}}}
%\def\iotadd{\ddot{{\iota}}}
%\def\kappadd{\ddot{{\kappa}}}
%\def\lambdadd{\ddot{{\lambda}}}
%\def\mudd{\ddot{{\mu}}}
%\def\nudd{\ddot{{\nu}}}
%\def\pidd{\ddot{{\pi}}}
%\def\rhodd{\ddot{{\rho}}}
%\def\sigmadd{\ddot{{\sigma}}}
%\def\taudd{\ddot{{\tau}}}
%\def\upsilondd{\ddot{{\upsilon}}}
%\def\phidd{\ddot{{\phi}}}
%\def\chidd{\ddot{{\chi}}}
%\def\psidd{\ddot{{\psi}}}
%\def\omegadd{\ddot{{\omega}}}
%\def\Gammadd{\ddot{{\Gamma}}}
%\def\Deltadd{\ddot{{\Delta}}}
%\def\Thetadd{\ddot{{\Theta}}}
%\def\Lambdadd{\ddot{{\Lambda}}}
%\def\Pidd{\ddot{{\Pi}}}
%\def\Sigmadd{\ddot{{\Sigma}}}
%\def\Upsilondd{\ddot{{\Upsilon}}}
%\def\Phidd{\ddot{{\Phi}}}
%\def\Psidd{\ddot{{\Psi}}}
%\def\Omegadd{\ddot{{\Omega}}}
%
%
%
%
%
%

